Towards Realistic Statistical Channel Models For Positioning: Evaluating the Impact of Early Clusters

Physical effects such as reflection, refraction, and diffraction cause a radio signal to arrive from a transmitter to a receiver in multiple replicas that have different amplitude and rotation. Bandwidth-limited signals, such as positioning reference signals, have a limited time resolution. In reality, the signal is often reflected in the close vicinity of a transmitter and receiver, which causes the displacement of the observed peak from the true peak expected according to the line of sight (LOS) geometry between the transmitter and receiver. In this paper, we show that the existing channel model specified for performance evaluation within 3GPP fails to model the above phenomena. As a result, the simulation results deviate significantly from the measured values. Based on our measurement and simulation results, we propose a model for incorporating the signal reflection by obstacles in the vicinity of transmitter or receiver, so that the outcome of the model corresponds to the measurement made in such scenario.

==> src/__3gppmodels.tex <==
\section{Review of 3GPP channel model in the context of positioning systems}
\subsection{Positioning properties expected based on TR38.901 }
Basic model (issues we discussed on multiple occasions) on LOS and NLOS channels including  the ATOA extensions of the Inf models

\subsection{Impact on the positioning evaluations}
Optimistic Estimates due to the low probability of early clusters 

==> src/__evaluation.tex <==
\section{Evaluation}
% some results showing how the observation measurement are covered by the model

\noindent
For the evaluation of the proposed method we rebuild the setups of the experiments described in section ~\ref{sec:ObservationMeasurements} in simulation using the SDC concept. 


The channel generated in simulation included three parts,
\begin{itemize}
\item Statistical part using 3GPP InF-LOS parameter set
\item SDC representing the room cube (walls, ceiling, floor). Specular reflection was assumed for these objects. The position of the effective scatterer position was calculated according the UE position. 
\item SDC representing objects close to the UE. The position of these objects was selected randomly and was fixed for different UE positions (heights). 
\end{itemize}


%% Bild aus WordDocument, ??? ADD legend, change text size
%\begin{figure}[htbp]
%\centering
%\includegraphics[width=1.0\columnwidth] {figures/MovingBlockerSimulation.png}
%\caption{Simulated power for diffraction experiment using SDC}\label{fig:MovingBlockerSimulation}
%\end{figure}    



